MM-BRIGHT: A Multi-Task Multimodal Benchmark for Reasoning-Intensive Retrieval

Existing retrieval benchmarks primarily consist of text-based queries where keyword or semantic matching is usually sufficient. Many real-world queries contain multimodal elements, particularly, images such as diagrams, charts, and screenshots that require intensive reasoning to identify relevant documents. To address this gap, we introduce MM-BRIGHT, the first multimodal benchmark for reasoning-intensive retrieval. Our dataset consists of 2,803 real-world queries spanning 29 diverse technical domains, with four tasks of increasing complexity: text-to-text, multimodal-to-text, multimodal-to-image, and multimodal-to-multimodal retrieval. Extensive evaluation reveals that state-of-the-art models struggle across all tasks: BM25 achieves only 8.5 nDCG@10 on text-only retrieval, while the best multimodal model Nomic-Vision reaches just 27.6 nDCG@10 on multimodal-to-text retrieval actually underperforming the best text-only model (DiVeR: 32.2). These results highlight substantial headroom and position MM-BRIGHT as a testbed for next-generation retrieval models that better integrate visual reasoning. Our code and data are available at https://github.com/mm-bright/MM-BRIGHT. See also our official website: https://mm-bright.github.io/.

==> figures/image_essentiality_charts/essentiality_table.tex <==
\begin{table}[t]
\centering
\caption{Image essentiality distribution across domains in MM-BRIGHT. We classify images as \textit{essential} (critical for understanding the query), \textit{helpful} (provides useful context), or \textit{redundant} (not necessary for retrieval).}
\label{tab:image_essentiality}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|r|rrr}
\toprule
\textbf{Domain} & \textbf{Queries} & \textbf{Essential} & \textbf{Helpful} & \textbf{Redundant} \\
\midrule
\rowcolor{gray!12}\multicolumn{5}{c}{\textit{STEM \& Life Sciences}} \\
\midrule
Biology & 64 & 34 & 28 & 2 \\
Chemistry & 51 & 22 & 26 & 3 \\
Physics & 79 & 21 & 52 & 6 \\
Math & 38 & 16 & 22 & 0 \\
Earthscience & 71 & 15 & 45 & 10 \\
Bioacoustics & 39 & 22 & 16 & 1 \\
Bioinformatics & 46 & 20 & 26 & 0 \\
Medicalsciences & 43 & 14 & 22 & 7 \\
\midrule
\rowcolor{gray!12}\multicolumn{5}{c}{\textit{Software \& Technical}} \\
\midrule
Ubuntu & 27 & 4 & 21 & 2 \\
Bitcoin & 54 & 13 & 40 & 1 \\
Crypto & 51 & 16 & 31 & 4 \\
Quantumcomputing & 64 & 37 & 27 & 0 \\
Robotics & 23 & 5 & 16 & 2 \\
Salesforce & 8 & 2 & 5 & 1 \\
Apple & 13 & 2 & 10 & 1 \\
Gis & 34 & 12 & 19 & 3 \\
\midrule
\rowcolor{gray!12}\multicolumn{5}{c}{\textit{Social Sciences}} \\
\midrule
Economics & 28 & 9 & 19 & 0 \\
Psychology & 46 & 12 & 27 & 7 \\
Philosophy & 38 & 6 & 29 & 3 \\
Law & 23 & 2 & 14 & 7 \\
Christianity & 22 & 4 & 16 & 2 \\
Islam & 24 & 7 & 10 & 7 \\
\midrule
\rowcolor{gray!12}\multicolumn{5}{c}{\textit{Applied Domains}} \\
\midrule
Aviation & 111 & 25 & 70 & 16 \\
Gaming & 19 & 5 & 9 & 5 \\
Project Mgmt & 42 & 13 & 27 & 2 \\
Quant & 28 & 9 & 17 & 2 \\
Sustainability & 53 & 6 & 36 & 11 \\
Travel & 45 & 15 & 24 & 6 \\
Academia & 22 & 8 & 11 & 3 \\
\midrule
\textbf{Total} & \textbf{1206} & \textbf{376} & \textbf{715} & \textbf{114} \\
\bottomrule
\end{tabular}}
\end{table}

==> figures/image_type_charts/image_type_table.tex <==
\begin{table*}[t]
\centering
\caption{Image type distribution across domains in MM-BRIGHT}
\label{tab:image_type_distribution}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|r|rrrrrrrr}
\toprule
\textbf{Domain} & \textbf{Total} & \rotatebox{45}{\textbf{Diagrams}} & \rotatebox{45}{\textbf{Screenshots}} & \rotatebox{45}{\textbf{Charts/Graphs}} & \rotatebox{45}{\textbf{Photos}} & \rotatebox{45}{\textbf{Mathematical}} & \rotatebox{45}{\textbf{Scientific Fig.}} & \rotatebox{45}{\textbf{Mixed}} & \rotatebox{45}{\textbf{Other}} \\
\midrule
Aviation & 262 & 35 & 9 & 9 & 197 & 2 & 5 & 3 & 2 \\
Physics & 198 & 67 & 4 & 21 & 54 & 12 & 28 & 1 & 11 \\
Biology & 188 & 7 & 0 & 16 & 128 & 0 & 30 & 1 & 6 \\
Earthscience & 156 & 19 & 3 & 36 & 37 & 5 & 50 & 4 & 2 \\
Chemistry & 124 & 12 & 0 & 9 & 5 & 12 & 83 & 1 & 2 \\
Quantumcomputing & 113 & 69 & 3 & 6 & 0 & 21 & 5 & 7 & 2 \\
Math & 107 & 7 & 2 & 31 & 5 & 49 & 7 & 2 & 4 \\
Gis & 94 & 26 & 38 & 11 & 0 & 4 & 10 & 3 & 2 \\
Sustainability & 88 & 12 & 0 & 11 & 55 & 1 & 0 & 1 & 8 \\
Bioacoustics & 86 & 4 & 37 & 20 & 2 & 1 & 21 & 0 & 1 \\
Travel & 82 & 4 & 12 & 0 & 59 & 0 & 0 & 0 & 7 \\
Bitcoin & 79 & 13 & 39 & 18 & 0 & 7 & 0 & 2 & 0 \\
Medicalsciences & 76 & 11 & 2 & 10 & 29 & 0 & 18 & 1 & 5 \\
Crypto & 75 & 32 & 4 & 8 & 2 & 25 & 0 & 1 & 3 \\
Bioinformatics & 72 & 10 & 8 & 44 & 0 & 0 & 8 & 2 & 0 \\
Pm & 70 & 23 & 33 & 11 & 1 & 0 & 0 & 1 & 1 \\
Psychology & 69 & 13 & 5 & 24 & 13 & 1 & 8 & 1 & 4 \\
Robotics & 63 & 28 & 2 & 9 & 20 & 2 & 1 & 1 & 0 \\
Askubuntu & 61 & 1 & 58 & 0 & 1 & 0 & 0 & 0 & 1 \\
Philosophy & 57 & 7 & 3 & 6 & 2 & 23 & 5 & 0 & 11 \\
Economics & 53 & 2 & 2 & 44 & 1 & 3 & 0 & 0 & 1 \\
Quant & 38 & 1 & 1 & 28 & 0 & 7 & 0 & 0 & 1 \\
Gaming & 37 & 1 & 19 & 2 & 3 & 0 & 0 & 0 & 12 \\
Christianity & 33 & 3 & 0 & 1 & 9 & 0 & 0 & 0 & 20 \\
Islam & 33 & 1 & 5 & 1 & 15 & 0 & 0 & 0 & 11 \\
Law & 30 & 2 & 8 & 1 & 17 & 0 & 0 & 0 & 2 \\
Apple & 29 & 0 & 25 & 1 & 1 & 0 & 0 & 1 & 1 \\
Academia & 28 & 1 & 5 & 12 & 2 & 2 & 1 & 0 & 5 \\
Salesforce & 21 & 4 & 9 & 0 & 0 & 8 & 0 & 0 & 0 \\
\midrule
\textbf{Total} & \textbf{2422} & \textbf{415} & \textbf{336} & \textbf{390} & \textbf{658} & \textbf{185} & \textbf{280} & \textbf{33} & \textbf{125} \\
\bottomrule
\end{tabular}}
\end{table*}
